StructEdit: Learning Structural Shape Variations

Learning to encode differences in the geometry and (topological) structure of the shapes of ordinary objects is key to generating semantically plausible variations of a given shape, transferring edits from one shape to another, and many other applications in 3D content creation. The common approach of encoding shapes as points in a high-dimensional latent feature space suggests treating shape differences as vectors in that space. Instead, we treat shape differences as primary objects in their own right and propose to encode them in their own latent space. In a setting where the shapes themselves are encoded in terms of fine-grained part hierarchies, we demonstrate that a separate encoding of shape deltas or differences provides a principled way to deal with inhomogeneities in the shape space due to different combinatorial part structures, while also allowing for compactness in the representation, as well as edit abstraction and transfer. Our approach is based on a conditional variational autoencoder for encoding and decoding shape deltas, conditioned on a source shape. We demonstrate the effectiveness and robustness of our approach in multiple shape modification and generation tasks, and provide comparison and ablation studies on the PartNet dataset, one of the largest publicly available 3D datasets.

==> tex/overview.tex <==
Our goal is to create a latent space of shape edits.

A shape $A$ is defined as a hierarchy of parts, where each part is defined by its oriented bounding box. A shape edit $E_A$ maps a shape $A$ to an edited shape $A'$. It is defined as a hierarchy of part edits, using the same hierarchical structure as $A$, except for the set of parts that are newly created by the edit; these parts are added as new nodes to the hierarchy. Each node in the edit describes what happens to the corresponding shape part during an edit. The part can either be \emph{deleted}, \emph{modified}, or newly \emph{created}. In the latter two cases, the edit node stores the modification to the bounding box parameters, or the new bounding box parameters. See Figure~\ref{fig:edit_hierarchy} for an illustration.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/edit.png}
    \caption{The part hierarchy of a shape (left) and a corresponding hierarchy of part edits (right).}
    \label{fig:edit_hierarchy}
\end{figure}

The set of edits we would like to encode is defined by a dataset of shapes $\mathbf{S}$ and a definition of a neighborhood $\mathbf{N}$ around each shape $A \in \mathbf{S}$. The neighborhood could, for example, be defined by the n-nearest neighbors (or all shapes inside a given radius) under the chamfer distance, a structural distance, the L2 distance in a latent space encoding of the dataset $\mathbf{S}$, etc. Our goal is to encode a set of edits that allows us to reach each neighbor of a shape, for all shapes in the dataset.

The neighborhoods are different for each shape $A$, but we assume that there are (semantic) commonalities among the edits in each neighborhood. For example, many neighborhoods of chairs will have edits to stretch/shorten the backrest or the legs. We want to encode the edits for all shapes into a common latent space $\mathcal{L}$, where similar edits can be encoded into similar vectors:
\begin{equation}
z_E = e(E_A, A),
\end{equation}
where $z_E \in \mathcal{L}$ is the latent feature representation of an the $E$ that is now independent of the input shape. This latent space contains a superset of edits that are not necessarily directly applicable to all shapes in the dataset. To describe the edits that are directly applicable to a different shape $B$, we create a second smaller latent space $\mathcal{L}_{B}$ that is conditioned on $B$. We adapt global edits to a shape by mapping them from  $\mathcal{L}$ to $\mathcal{L}_{B}$ with a network $a$ that is conditioned on $B$:
\begin{equation}
z_{E_{B}} = a(z_E, B),
\end{equation}
where $z_{E_{B}} \in \mathcal{L}_{B}$ is the feature representation of the adapted edit. The adapted edit feature vector can then be decoded using a conditional decoder:
\begin{equation}
E_B = d(z_{E_{B}}, B),
\end{equation}
giving us the edit $E_A$ transferred to shape $B$.
